3-D Motion Capture of an Unmodified Drone with Single-chip Millimeter Wave Radar

Accurate motion capture of aerial robots in 3-D is a key enabler for autonomous operation in indoor environments such as warehouses or factories, as well as driving forward research in these areas. The most commonly used solutions at present are optical motion capture (e.g. VICON) and Ultrawideband (UWB), but these are costly and cumbersome to deploy, due to their requirement of multiple cameras/sensors spaced around the tracking area. They also require the drone to be modified to carry an active or passive marker. In this work, we present an inexpensive system that can be rapidly installed, based on single-chip millimeter wave (mmWave) radar. Importantly, the drone does not need to be modified or equipped with any markers, as we exploit the Doppler signals from the rotating propellers. Furthermore, 3-D tracking is possible from a single point, greatly simplifying deployment. We develop a novel deep neural network and demonstrate decimeter level 3-D tracking at 10Hz, achieving better performance than classical baselines. Our hope is that this low-cost system will act to catalyse inexpensive drone research and increased autonomy.

==> sections/background.tex <==
\section{mmWave Radar Background}
\label{sec_background}
%\subsection{Millimeter Wave FMCW Radar}
\subsection{Range Measurement}
Millimeter Wave (mmWave) Radar follows FMCW radar design principle, and uses short-wavelength electromagnetic waves. Transmitter in the radar system transmits chirps, which are short period signals with increasing frequency. The signals are received by co-located receiver after reflecting from objects. A mixer mixes the receiving signal and the transmitting signal, producing IF signal, from which we can estimate the distance to the object. As the frequency of the transmitting signal is linearly increasing, the further away the object, the bigger frequency difference there will be between the transmitting signal and receiving signal, resulting in a higher frequency component in the IF signal. For each frequency component, the range of the corresponding object can be extracted as:
\begin{equation}
    d=\frac{f_{IF}c}{2S}
\end{equation}
where $f_{IF}$ is the frequency of each component of the IF signal, $c$ represents the speed of light, and $S$ is the frequency slope of the chirp.
As a result, we can extract the range to different objects by performing a Fast-Fourier Transform (FFT) on the IF signal. This process is called `Range FFT'.

\subsection{Speed Detection}
A frame is formed by a series of consecutive chirps. If the target has a relative radial speed to the sensor, the phase of the corresponding peak in the range profile generated with Range FFT would change across chirps. The speed can estimated with:
\begin{equation}
    v=\frac{\lambda \Delta \phi}{4\pi T_{c}}
\end{equation}
where $lambda$ is the wavelength of the signal, $\Delta \phi$ is the phase difference between two chirps, and $T_{c}$ is the time of a chirp.
We can perform a FFT along the chirp dimension, and estimate the speed with the phase difference extracted from the FFT algorithm. This process is often called `velocity FFT', which can be performed on every point in the range profile. After velocity FFT, we can have a range-velocity heatmap of size $Nc * Ns$, where $Nc$ is the chirp number in a frame, and $Ns$ is the sample number of each chirp. The peak in the range-velocity heatmap corresponding to objects with certain distance and radial speeds.

\subsection{Angle Estimation}
The phase of the receiving signal reflected from the same object at a pair of receivers can have a phase difference, due to the distance between the receivers. As we know the distance between each pair of receivers, we can estimate the angle of arrival, and thus compute the location of the object along with the range information. The angle of arrival can be calculated as:
\begin{equation}
\theta=sin^{-1}(\frac{\lambda \omega}{2\pi d})
\end{equation}
where $\lambda$ is the wavelength of the signal, $\omega$ is the phase difference and $d$ is the distance of the two receiver antennas.
In the Multi-Input Multi-Output (MIMO) radar which we use in this project, we can perform a FFT on the virtual antenna array to estimate the angle of arrival for each object. This process is called `Angle FFT'.

%\subsection{Conventional Drone Tracking Pipeline}


==> sections/data.tex <==
\section{Data Collection}
\label{sec_data_acq}
\subsection{Data Collection Setup}
We collected 100 1-minute long sequences of drone randomly flying in a room equipped with Vicon system which provides ground truth. For each sequence, the data collection begins after the drone is launched into the air so the 100 sequences contains purely the data of the drone flying around.

\begin{table}[h!]
  \begin{center}
    \caption{mmWave Radar Configuration.}
    \label{tab:config}
    \begin{tabular}{l|c|r} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \textbf{Value 1} & \textbf{Value 2} & \textbf{Value 3}\\
      $\alpha$ & $\beta$ & $\gamma$ \\
      \hline
      1 & 1110.1 & a\\
      2 & 10.1 & b\\
      3 & 23.113231 & c\\
    \end{tabular}
  \end{center}
\end{table}

We use IWR6843ISK\footnote{\url{http://www.ti.com/tool/IWR6843ISK}} together with DCA1000EVM\footnote{\url{http://www.ti.com/tool/DCA1000EVM}} for raw data streaming. The configuration of the mmWave radar is shown in Table.~\ref{tab:config}. A desktop computer with Windows operating system is used for configuring the device and recording raw radar data, with mmWave Studio software\footnote{\url{http://www.ti.com/tool/MMWAVE-STUDIO}}. The raw data file is parsed and saved frame by frame. A laptop with Ubuntu operating system and ROS is used for Vicon data recording, and the Vicon data is later parsed to extract ground truth. 

\subsection{Time Synchronization}
Since the raw data streaming and Vicon data recording happen on two platforms respectively, we need to synchronize the timestamps of each frame in mmWave data to the corresponding Vicon ground truth. The time of the two platforms are synchronized using NTP server. mmWave Studio is not able to provide timestamp logging for each frame, so we record the time when the radar starts and extrapolate the timestamp of each frame based on frame period. 

\subsection{Ground Truth Generation}
We attach two Vicon markers on the mmWave radar and the drone respectively, as shown in Fig.~\ref{fig:setup}. The pose of the drone and the mmWave sensor are relative poses to the Vicon system, and the orientation of each marker is randomly assigned when creating the marker. The drone pose we are trying to predict is the relative pose to the mmWave radar. As a result, we need to convert the pose data to the coordinate system of mmWave radar.


